Strange Quark Contribution to the Nucleon - (Dissertation)

The strangeness contribution to the electric and magnetic properties of the nucleon has been under investigation experimentally for many years. Lattice Quantum Chromodynamics (LQCD) gives theoretical predictions of these measurements by implementing the continuum gauge theory on a discrete, mathematical Euclidean space-time lattice which provides a cutoff removing the ultra-violet divergences. In this dissertation we will discuss effective methods using LQCD that will lead to a better determination of the strangeness contribution to the nucleon properties. Strangeness calculations are demanding technically and computationally. Sophisticated techniques are required to carry them to completion. In this thesis, new theoretical and computational methods for this calculation such as twisted mass fermions, perturbative subtraction, and General Minimal Residual (GMRES) techniques which have proven useful in the determination of these form factors will be investigated. Numerical results of the scalar form factor using these techniques are presented. These results give validation to these methods in future calculations of the strange quark contribution to the electric and magnetic form factors.

==> diss.bib.tex <==
%%%
%%% Bibliography for Dissertation by John Perkins
%%%
%revit
@Article{Kuck,
     author    = "A.H. Sameh and D.J. Kuck",
     title     = "On Stabel Parallel Linear System Solvers",
     journal   = "Journal of the ACM (JACM)",
     volume    = "25 Issue 1",
     year      = "1978",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%BEGIN TOGETHER

@Book{Golub,
     author    = "Gene H. Golub and Charles F. van Loan",
     title     = "Matrix Computations",
     year      = "1989",
     pages     = "",
     publisher = "The Johns Hopkins University Press",
     city      = ""
}

@Book{Saadeval,
     author    = "Yousef Saad",
     title     = "Numerical Methods For Large Eigenvalue Problems",
     year      = "1992",
     pages     = "175-176",
     publisher = "Manchester University Press",
     city      = "New York"
}

@Book{Saad,
     author    = "Yousef Saad",
     title     = "Iterative Methods for Sparce Linear Systems",
     year      = "2003",
     pages     = "153",
     publisher = "Society of Industrial and Applies Mathematics (SIAM)",
     city      = "Philadelphia, PA"
}

@Article{Harmonic,
     author    = "Ronald Morgan and M. Zeng",
     title     = "Harmonic projection methods for large non-symmetric eigenvalue problems",
     journal   = "Num. Lin. Alg. with Appl.",
     volume    = "5:33-55",
     year      = "1998",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{Harmonic1,
     author    = "Ronald B.Morgan",
     title     = "Computing interior eigenvalues of large matricies",
     journal   = "Linear Algebra Appl.",
     volume    = "154-156:289-309",
     year      = "1991",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{Harmonic2,
     author    = "C.C. Paige and B.N. Parlett and H.A. van der Vorst",
     title     = "Approximate solutions and eigenvalue bounds from Krylov subspaces",
     journal   = "Num. Lin. Alg. with Appl.",
     volume    = "2:115-133",
     year      = "1995",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{Harmonic3,
     author    = "Ronald Morgan and M. Zeng",
     title     = "A Jacobi-Davidson iteration method for linear eigenvalue problems",
     journal   = "SIAM J. Matrix Anal. Appl.",
     volume    = "17:401-425",
     year      = "1996",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{GMRESDR,
     author    = "Ronald B. Morgan",
     title     = "GMRES with Deflated Restarting",
     journal   = "SIAM Journal of Scientific Computing",
     volume    = "Volume 24, Number 1",
     year      = "2002",
     pages     = "20-37",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{evalDR,
     author    = "Ronald B. Morgan and Walter Wilcox",
     title     = "Deflation of Eigenvalues for GMRES in Lattice QCD",
     journal   = "Nucl..Phys.Proc.Suppl",
     volume    = "Volume 106",
     year      = "2002",
     pages     = "1067-1069",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{implicit,
     author    = "Ronald B. Morgan",
     title     = "Implicitly Restarted GMRES and Arnoldi Methods for Nonsymmetric Systems of Equations",
     journal   = "SIAM J. Matrix Anal. Appl.",
     volume    = "Volume 17",
     year      = "1996",
     pages     = "401-425",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{Harmonic4,
     author    = "G.L.G Sleijpen and H.A. van der Vorst",
     title     = "A Jacobi-Davidson Iteration Method for Linear Eigenvalue Problems",
     journal   = "SIAM J. Matrix Anal. Appl.",
     volume    = "Volume 24, Number 4",
     year      = "2000",
     pages     = "1112-1135",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}

==> diss.tex <==
%%%
%%% Bibliography for Dissertation by John Perkins
%%%
%revit
@Article{Kuck,
     author    = "A.H. Sameh and D.J. Kuck",
     title     = "On Stabel Parallel Linear System Solvers",
     journal   = "Journal of the ACM (JACM)",
     volume    = "25 Issue 1",
     year      = "1978",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%BEGIN TOGETHER

@Book{Golub,
     author    = "Gene H. Golub and Charles F. van Loan",
     title     = "Matrix Computations",
     year      = "1989",
     pages     = "",
     publisher = "The Johns Hopkins University Press",
     city      = ""
}

@Book{Saadeval,
     author    = "Yousef Saad",
     title     = "Numerical Methods For Large Eigenvalue Problems",
     year      = "1992",
     pages     = "175-176",
     publisher = "Manchester University Press",
     city      = "New York"
}

@Book{Saad,
     author    = "Yousef Saad",
     title     = "Iterative Methods for Sparce Linear Systems",
     year      = "2003",
     pages     = "153",
     publisher = "Society of Industrial and Applies Mathematics (SIAM)",
     city      = "Philadelphia, PA"
}

@Article{Harmonic,
     author    = "Ronald Morgan and M. Zeng",
     title     = "Harmonic projection methods for large non-symmetric eigenvalue problems",
     journal   = "Num. Lin. Alg. with Appl.",
     volume    = "5:33-55",
     year      = "1998",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{Harmonic1,
     author    = "Ronald B.Morgan",
     title     = "Computing interior eigenvalues of large matricies",
     journal   = "Linear Algebra Appl.",
     volume    = "154-156:289-309",
     year      = "1991",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{Harmonic2,
     author    = "C.C. Paige and B.N. Parlett and H.A. van der Vorst",
     title     = "Approximate solutions and eigenvalue bounds from Krylov subspaces",
     journal   = "Num. Lin. Alg. with Appl.",
     volume    = "2:115-133",
     year      = "1995",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{Harmonic3,
     author    = "Ronald Morgan and M. Zeng",
     title     = "A Jacobi-Davidson iteration method for linear eigenvalue problems",
     journal   = "SIAM J. Matrix Anal. Appl.",
     volume    = "17:401-425",
     year      = "1996",
     pages     = "",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{GMRESDR,
     author    = "Ronald B. Morgan",
     title     = "GMRES with Deflated Restarting",
     journal   = "SIAM Journal of Scientific Computing",
     volume    = "Volume 24, Number 1",
     year      = "2002",
     pages     = "20-37",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{evalDR,
     author    = "Ronald B. Morgan and Walter Wilcox",
     title     = "Deflation of Eigenvalues for GMRES in Lattice QCD",
     journal   = "Nucl..Phys.Proc.Suppl",
     volume    = "Volume 106",
     year      = "2002",
     pages     = "1067-1069",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{implicit,
     author    = "Ronald B. Morgan",
     title     = "Implicitly Restarted GMRES and Arnoldi Methods for Nonsymmetric Systems of Equations",
     journal   = "SIAM J. Matrix Anal. Appl.",
     volume    = "Volume 17",
     year      = "1996",
     pages     = "401-425",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
@Article{Harmonic4,
     author    = "G.L.G Sleijpen and H.A. van der Vorst",
     title     = "A Jacobi-Davidson Iteration Method for Linear Eigenvalue Problems",
     journal   = "SIAM J. Matrix Anal. Appl.",
     volume    = "Volume 24, Number 4",
     year      = "2000",
     pages     = "1112-1135",
     SLACcitation  = "%%CITATION = PHLTA,B194,231;%%"
}
